First measurement of the Sivers asymmetry for gluons from SIDIS data

The Sivers function describes the correlation between the transverse spin of a nucleon and the transverse motion of its partons. It was extracted from measurements of the azimuthal asymmetry of hadrons produced in semi-inclusive deep inelastic scattering of leptons off transversely polarised nucleon targets, and it turned out to be non-zero for quarks. In this letter the evaluation of the Sivers asymmetry for gluons in the same process is presented. The analysis method is based on a Monte Carlo simulation that includes three hard processes: photon-gluon fusion, QCD Compton scattering and leading-order virtual-photon absorption process. The Sivers asymmetries of the three processes are simultaneously extracted using the LEPTO event generator and a neural network approach. The method is applied to samples of events containing at least two hadrons with large transverse momentum from the COMPASS data taken with a 160 GeV/$c$ muon beam scattered off transversely polarised deuterons and protons. With a significance of more than two standard deviations a negative value is obtained for the gluon Sivers asymmetry. The result of a similar analysis for a Collins-like asymmetry for gluons is consistent with zero.

==> mean_asymmetry.tex <==
\section{Mean asymmetry}
\label{sect:app}
The mean asymmetry as in Eqs. \ref{eq:weighted_processes} and \ref{eq:beta} is given by
\begin {equation}
\big\{A_{Sivers}(\vec{x})\big\}_{\beta\omega}=\frac{\int d\vec{x}d\phi_{Sivers} A_{Sivers}(\vec{x})\omega(\phi_{Sivers})\beta_t(\phi_{Sivers})\alpha_t(\vec{x}, \phi_{Sivers})}{\int d\vec{x}d\phi_{Sivers}\omega(\phi_{Sivers})\beta_t(\phi_{Sivers})\alpha_t(\vec{x}, \phi_{Sivers})}.
\end{equation}
Introducing $\vec{x'}=(Q^2, p_{T1}, p_{T2}, z_1, z_2)$ ($\vec{x}=(x_{Bj}, \vec{x'})$) and assuming linearity in $x_{Bj}$ (or $x_g$ or $x_C$) it means $A_{Sivers}=a(\vec{x'})(x_{Bj}-\langle x_{Bj} \rangle) + A_{Sivers}(\langle x_Bj \rangle)$ the above equation reads 
\begin {equation}
\big\{A_{Sivers}(\vec{x})\big\}_{\beta\omega}=A_{Sivers}(\langle x_Bj \rangle),
\end{equation}
when
\begin{equation} 
   \langle x_{Bj}\rangle_{\omega\beta} \equiv\frac{\int d\vec{x}d\phi_{Sivers}a(\vec{x'})\alpha_t(\vec{x},\phi_{Sivers})x_{Bj}\omega(\phi_{Sivers})\beta(\phi_{Sivers})}{\int d\vec{x}d\phi_{Sivers}a(\vec{x'})\alpha_t(\vec{x},\phi_{Sivers})\omega(\phi_{Sivers})\beta(\phi_{Sivers})}\approx \frac{\sum_{i} x^i_{Bj}\beta^i \omega_i}{\sum_{i}\beta_i\omega_i}.
\end {equation}
The last approximation assumes that the raw asymmetries are small $\beta A_{Sivers}\ll 1$. 

